When Vision Becomes Text: Visual Token Pruning via Cross-Modal Residual Guidance in VLMs

Abundant visual information strengthens vision-language model (VLM) perception, yet massive visual tokens raise inference costs. Existing visual token pruning methods rely on similarity-based guidance, which exploits pairwise text-vision and vision-vision token correlations for compression. However, such methods only capture local layer-level signals and overlook the whole inference process in VLM. In this paper, we revisit VLM inference and present a new efficient guidance scheme that complements similarity-based guidance. In particular, we identify a key observation: as LLM layers deepen, text tokens continuously aggregate visual information via self-attention and progressively absorb partial visual content into textual representations. To quantify this phenomenon, we propose Cross Modal Absorption (CMA) from a geometric representation perspective to measure how much visual information is absorbed by text, revealing that more visual tokens in deeper layers can be approximately explained by the text subspace. We accordingly propose Cross Modal Residual (CMR). It projects visual tokens onto the text subspace via Tikhonov regularized least squares and exploits reconstruction residuals to quantify visual information that cannot be explained by text. Finally, based on CMR, we present SIEVE, a training-free visual token compression method that combines CMR, text-attention relevance, and residual-space diversity to retain task-relevant and complementary tokens. Experiments on diverse VLM architectures verify the effectiveness of SIEVE. For instance, on LLaVA-NeXT-7B, SIEVE keeps only $11.1\%$ of visual tokens while preserving $97.5\%$ of the original average performance, achieving $3.62\times$ prefill speedup, $2.49\times$ end-to-end speedup, and a $6.02\times$ KV-cache reduction.

==> Sections_Analysis.tex <==
% \section{Analysis}
% \label{sec:analysis}

% Existing methods mainly select tokens based on current-layer attention or feature similarity, but such criteria only reflect the local state at a single layer and lack a view of the whole multimodal reasoning process, making it difficult to accurately assess the necessity of retaining visual tokens. To this end, we step beyond the single-layer view and revisit the inference process of VLMs, examining the geometric relationship between visual tokens and the text representation space: as the model goes deeper, do visual tokens remain relatively independent, or are they progressively absorbed by the text subspace?

% We analyze all 32 layers of LLaVA-1.5-7B on three benchmarks, TextVQA~\cite{singh2019textvqa}, POPE~\cite{li2023pope}, and MME~\cite{fu2025mme}, covering 16,284 samples. The results show that an increasing portion of visual-token representations can be explained by the text subspace, indicating that visual information is progressively integrated into the text representation space during forward propagation.

% \subsection{Measuring Cross Modal Absorption}
% \label{sec:measuring_cma}
% To quantify this phenomenon, we define \textbf{Cross Modal Absorption (CMA)} to measure how much of the visual token representation at a given layer can be explained by the text subspace. The CMA at layer $l$ is defined as
% \begin{equation}
% \mathrm{CMA}=
% 1 -
% \frac{
% \left\|
% V_c - \hat{V}_c
% \right\|_F^2
% }{
% \left\|
% V_c
% \right\|_F^2
% }.
% \end{equation}
% Here, $V_c$ denotes the matrix of all centered visual tokens at layer $l$ (rather than an individual token); $\hat{V}_c$ denotes its projection onto the text subspace; and $||\cdot||_F$ denotes the Frobenius norm. CMA is thus a layer-level metric: a larger value indicates that more visual information can be explained by the text subspace, i.e., stronger cross modal absorption. 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.4\textwidth]{Images/cma_kurt_left.pdf}
%     \caption{
% Layer-wise evolution of Cross-modal absorption in LLaVA-1.5-7B.
% Cross-modal absorption (CMA) increases across Transformer layers.
%     }
%     \label{fig:cma_kurt}
% \end{figure}

% \subsection{Visual Tokens Are Progressively Absorbed by the Text Subspace}
% \label{sec:cma_results}

% As shown in Fig.~\ref{fig:cma_kurt}, CMA consistently increases from shallow to deep layers across all three benchmarks: from $0.008$ to $0.209$ on POPE, from $0.009$ to $0.217$ on MME, and from $0.017$ to $0.396$ on TextVQA. The Spearman correlation between CMA and layer depth reaches $\rho=+0.99$ on all three benchmarks, indicating a highly consistent monotonic trend.

% These results show that visual tokens do not remain fully independent throughout the network, but become increasingly explainable by the text subspace as depth grows. This can be understood as cross modal information flow in autoregressive VLMs: under causal attention, text tokens continuously aggregate visual information, so the text subspace comes to contain more visual-related directions. It also reveals cross modal redundancy in deep visual tokens: if a token can already be well explained by the text subspace, it may not need to be fully preserved. We can therefore measure, at the token level, the relationship between each visual token and the text subspace, preserving information that is difficult to explain by text while removing redundant tokens with little text-unexplained residual. Motivated by this, the next section introduces the token-level Cross-Modal Residual (CMR) and the CMR-based visual token compression algorithm, SIEVE.

% It is worth noting that the absolute value of CMA should not be interpreted directly on the $[0,1]$ scale. Since the number of text tokens is usually around $N_t \approx 30$, far smaller than the hidden dimension $D=4096$, a random subspace can theoretically explain only about $N_t/D \approx 0.007$ of a high-dimensional representation. Thus the final-layer CMA of $0.209$ on POPE is already about $29\times$ larger than the random baseline, indicating that the explanatory power of the text subspace over visual representations is not random but gradually emerges as a cross-modal representation pattern in deeper layers. Details are provided in Appendix B.


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.37\textwidth]{Images/cma_kurt_left.pdf}
    \caption{
Layer-wise evolution of cross-modal absorption in LLaVA-1.5-7B.
Cross-modal absorption (CMA) increases across Transformer layers.
    }
    \label{fig:cma_kurt}
\end{figure}


\section{Analysis}
\label{sec:analysis}

% Existing methods mainly select visual tokens based on current-layer attention or feature similarity. However, these criteria only capture the local state of a single layer and lack a holistic view of multimodal reasoning, making it difficult to determine whether a visual token still needs to be retained. We therefore step beyond the single-layer view and revisit the VLM inference process from a geometric perspective, examining the relationship between visual tokens and the text representation space: as layers go deeper, do visual tokens remain relatively independent, or are they progressively absorbed by the text subspace?

Differing from these works, we revisit the VLM inference process and investigate the evolution of visual tokens and text tokens throughout this procedure. Figure \ref{fig:cma_kurt} presents our observation. 


\begin{figure*}
    \centering
    \includegraphics[width=0.75\textwidth,height=0.45\textwidth,keepaspectratio]{Images/overall.pdf}
    \caption{
    Overview of SIEVE. SIEVE measures each visual token’s residual information with respect to the text subspace via CMR, combines it with attention relevance, and performs residual-space diversity selection to retain informative and non-redundant visual tokens for the compressed input sequence.
    }
    \label{fig:overall}
\end{figure*}


% Existing methods mainly select visual tokens based on current-layer attention or feature similarity. 

% However, these criteria only capture the local state of a single layer

% and lack a holistic view of multimodal reasoning, making it difficult to determine whether a visual token still needs to be retained. 

% We therefore step beyond the single-layer view and revisit the VLM inference process from a geometric perspective, examining the relationship between visual tokens and the text representation space: as layers go deeper, do visual tokens remain relatively independent, or are they progressively absorbed by the text subspace?

We analyze all 32 layers of LLaVA-1.5-7B on three benchmarks, TextVQA~\cite{singh2019textvqa}, POPE~\cite{li2023pope}, and MME~\cite{fu2025mme}, covering 16,284 samples. The results show that an increasing portion of visual-token representations can be explained by the text subspace, indicating that visual information is progressively integrated into the text representation space during forward propagation.



\subsection{Measuring Cross Modal Absorption}
\label{sec:measuring_cma}
To quantify this phenomenon, we define \textbf{Cross Modal Absorption (CMA)} to measure how much of the visual token representation at a given layer can be explained by the text subspace. The CMA at layer $l$ is defined as
\begin{equation}
\mathrm{CMA}=
1 -
\frac{
\left\|
V_c - \hat{V}_c
\right\|_F^2
}{
\left\|
V_c
\right\|_F^2
}.
\end{equation}
Here, $V_c$ denotes the matrix of all centered visual tokens at layer $l$ (rather than an individual token); $\hat{V}_c$ its projection onto the text subspace; and $||\cdot||_F$ the Frobenius norm. CMA is a layer-level metric: a larger value means more visual information can be explained by the text subspace, i.e., stronger cross modal absorption.


\subsection{Visual Tokens Are Progressively Absorbed by the Text Subspace}
\label{sec:cma_results}

As shown in Figure~\ref{fig:cma_kurt}, CMA consistently increases from shallow to deep layers across all three benchmarks: from $0.008$ to $0.209$ on POPE, from $0.009$ to $0.217$ on MME, and from $0.017$ to $0.396$ on TextVQA. Its Spearman correlation with layer depth reaches $\rho=+0.99$ on all three, indicating a highly consistent monotonic trend.

Thus visual tokens do not remain fully independent throughout the network, but become increasingly explainable by the text subspace as depth grows. This reflects cross modal information flow in autoregressive VLMs: under causal attention, text tokens continuously aggregate visual information, so the text subspace comes to contain more visual-related directions. \textbf{It also reveals cross modal redundancy in deep visual tokens: a token already well explained by the text subspace may not need to be fully preserved}. We can therefore measure, at the token level, the relationship between each visual token and the text subspace, keeping information that is hard to explain by text while removing redundant tokens with little text-unexplained residual. Accordingly, the next section introduces the token-level Cross-Modal Residual (CMR) and the CMR-based visual token compression algorithm, SIEVE.

Note that the absolute value of CMA should not be read directly on the $[0,1]$ scale. Since the number of text tokens is usually around $N_t \approx 30$, far smaller than the hidden dimension $D=4096$, a random subspace can theoretically explain only about $N_t/D \approx 0.007$ of a high-dimensional representation. Thus the final-layer CMA of $0.209$ on POPE is already about $29\times$ the random baseline, indicating that the explanatory power of the text subspace over visual representations is not random but gradually emerges as a cross-modal representation pattern in deeper layers. Details are provided in Appendix B.





==> Sections_Conclusion.tex <==
\section{Conclusion}\label{Conclusion}

% We revisit visual token retention in VLMs from the perspective of cross-modal reasoning dynamics, observing that text tokens progressively absorb visual information through self-attention as layers deepen. We propose CMA to quantify this absorption at the layer level and CMR to measure, at the token level, the unique visual information unexplained by text. Building on this, we design SIEVE, a training-free compression method that jointly leverages CMR, text-attention relevance, and residual-space diversity to retain tokens that are distinctive, task-relevant, and complementary, substantially reducing inference cost while preserving model performance.

In this work, we reveal cross-modal information absorption in VLMs and propose CMA for quantification. We design CMR via Tikhonov regularized subspace projection and develop the training-free SIEVE to compress visual tokens. Extensive evaluations over LLaVA, Qwen and LLaVA-NeXT verify that SIEVE substantially accelerates inference without obvious performance loss.

==> Sections_Experiments.tex <==




% Required packages:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table]{xcolor}

% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{2pt}

% \begin{tabular}{l|l|cccccccc|c}
% \toprule
% \textbf{Method} & \textbf{Venue}
% & \textbf{GQA} & \textbf{MMBench} & \textbf{MMBench-cn} & \textbf{MME}
% & \textbf{POPE} & \textbf{SQA} & \textbf{VQAv2} & \textbf{TextVQA}
% & \textbf{Avg} \\
% \midrule

% \rowcolor{HeaderGray}
% \textbf{LLaVA-NeXT-7B}
% &
% & \multicolumn{8}{c|}{\textbf{Upper Bound, 2880 Tokens}}
% & \\
% Vanilla & --
% & 64.2 & 67.4 & 60.6 & 1851 & 86.5 & 70.1 & 81.8 & 61.4
% & 100\% \\
% \midrule

% \rowcolor{HeaderGray}
% \textbf{LLaVA-NeXT-7B}
% &
% & \multicolumn{8}{c|}{\textbf{Retain 320 Tokens}}
% & \\
% FastV & ECCV'24
% & 55.9 & 61.6 & 51.9 & 1661 & 71.7 & 62.8 & 71.9 & 55.7
% & 88.1\% \\
% SparseVLM & ICML'25
% & 56.1 & 60.6 & 54.5 & 1533 & 82.4 & 66.1 & 71.5 & 58.4
% & 90.3\% \\
% VisionZip & CVPR'25
% & 59.3 & 63.1 & 55.6 & 1702 & 82.1 & 67.3 & 76.2 & 58.9
% & 93.7\% \\
% DART & EMNLP'25
% & 61.7 & 65.3 & 58.2 & 1710 & 84.1 & 68.4 & 79.1 & 58.7
% & 96.1\% \\
% HoloV & NeurIPS'25
% & 61.7 & 65.3 & 57.5 & 1738 & 83.9 & 68.9 & 79.5 & 58.7
% & 96.2\% \\
% SpecFlow & ICML'26
% & 62.5 & 66.7 & 56.8 & 1707 & 85.0 & 68.6 & 80.1 & 59.5
% & 96.6\% \\
% \rowcolor{OursBlue}
% SIEVE & Ours
% & 60.9 & 66.5 & 59.6 & 1819 & 85.7 & 68.3 & 78.7 & 59.6
% & \textbf{97.5\%} \\
% \bottomrule
% \end{tabular}%
% \caption{Performance comparison of different token reduction methods on LLaVA-NeXT-7B.}
% \label{tab:llava16_main}
% \end{table*}
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{2pt}

% \begin{tabular}{l|l|ccccccc|c}
% \toprule
% \textbf{Method} & \textbf{Venue}
% & \textbf{MMBench} & \textbf{MME} & \textbf{POPE} & \textbf{SQA}
% & \textbf{MMBench-cn} & \textbf{GQA} & \textbf{TextVQA} & \textbf{Avg} \\
% \midrule

% \rowcolor{HeaderGray}
% \textbf{Qwen2.5-VL-7B} &
% & \multicolumn{7}{c|}{\textbf{Upper Bound, 1296 Tokens}} & \\
% Vanilla & --
% & 83.4 & 2295 & 87.1 & 88.7 & 81.4 & 61.0 & 77.2 & 100.0\% \\
% \midrule

% \rowcolor{HeaderGray}
% \textbf{Qwen2.5-VL-7B} &
% & \multicolumn{7}{c|}{\textbf{Retain 33.3\% Tokens}} & \\
% FastV & ECCV'24
% & 79.5 & 2306 & 86.9 & 85.6 & 77.9 & 59.5 & 75.0 & 97.5\% \\
% HoloV & NeurIPS'25
% & 81.2 & 2288.9 & 86.1 & 88.7 & 80.0 & 60.2 & 74.4 & 98.5\% \\
% \rowcolor{OursBlue}
% SIEVE (Ours) & Ours
% & 82.5 & 2319 & 88.0 & 88.2 & 81.3 & 60.8 & 75.8 & \textbf{99.7\%} \\
% \midrule

% \rowcolor{HeaderGray}
% \textbf{Qwen2.5-VL-7B} &
% & \multicolumn{7}{c|}{\textbf{Retain 22.2\% Tokens}} & \\
% FastV & ECCV'24
% & 76.5 & 2243 & 85.1 & 84.8 & 75.2 & 57.8 & 73.5 & 95.0\% \\
% HoloV & NeurIPS'25
% & 80.5 & 2268.8 & 85.2 & 88.2 & 79.6 & 59.5 & 71.7 & 97.2\% \\
% \rowcolor{OursBlue}
% SIEVE (Ours) & Ours
% & 81.6 & 2313 & 87.3 & 87.5 & 80.2 & 60.3 & 75.1 & \textbf{98.9\%} \\
% \midrule

% \rowcolor{HeaderGray}
% \textbf{Qwen2.5-VL-7B} &
% & \multicolumn{7}{c|}{\textbf{Retain 11.1\% Tokens}} & \\
% FastV & ECCV'24
% & 71.2 & 2061 & 78.6 & 80.6 & 68.2 & 52.4 & 67.0 & 87.5\% \\
% HoloV & NeurIPS'25
% & 78.2 & 2246.5 & 83.7 & 87.6 & 77.1 & 57.5 & 65.7 & 94.4\% \\
% \rowcolor{OursBlue}
% SIEVE (Ours) & Ours
% & 80.0 & 2273 & 86.0 & 86.6 & 77.6 & 58.9 & 72.5 & \textbf{96.7\%} \\
% \bottomrule
% \end{tabular}%
% \caption{Performance comparison of different token reduction methods on Qwen2.5-VL-7B.}
% \label{tab:qwen2.5}
% \end{table*}
\section{Experiments}\label{Experiments}
\subsection{Experimental Setup}
\paragraph{Models and Baselines.}
We evaluate SIEVE on three VLMs of diverse architectures, including LLaVA-1.5~\cite{liu2023llava}, LLaVA-NeXT~\cite{liu2024llavanext}, and Qwen2.5-VL~\cite{bai2025qwen2}.

%and report results on eight widely adopted benchmarks.
% and compare it with eight representative visual-token reduction baselines: FastV~\cite{chen2024FastV}, SparseVLM~\cite{zhang2025sparsevlm}, VisionZip~\cite{yang2025visionzip}, DART~\cite{wen2025dart}, HoloV~\cite{holov}, SCOPE~\cite{deng2025scope},  and SpecFlow\cite{li2026spectral}.
\paragraph{Datasets. }
We report image-based results on eight standard benchmarks: GQA~\cite{hudson2019gqa}, MMBench and MMBench-CN~\cite{liu2024mmbench}, MME~\cite{fu2025mme}, POPE~\cite{li2023pope}, SQA~\cite{lu2022sqa}, VQAv2~\cite{goyal2017vqav2}, and TextVQA~\cite{singh2019textvqa}.
% \paragraph{Implementation Details. }
% We follow the default inference settings in the official codebases.
% The pruning layers are set to $[1,10,15]$ for LLaVA models and $[1,8,14]$ for Qwen models.
% For SIEVE, we set $\eta=0.75$ and $H_{\mathrm{top}}=12$.
\subsection{Comparison Experimental Results}

\noindent\textbf{Results on LLaVA.}
Table~\ref{tab:llava15_main} reports the results on LLaVA-1.5-7B.
Here, Vanilla denotes the original model without visual-token reduction.
On LLaVA-1.5-7B, SIEVE achieves the best average performance among methods with complete results under all token budgets.
With 192, 128, and 64 retained visual tokens, SIEVE preserves 99.1\%, 98.7\%, and 96.0\% of the Vanilla baseline, respectively.
Notably, even when retaining only 64 visual tokens, SIEVE still surpasses SCOPE, the strongest baseline with complete results, by 0.6 percentage points on average, demonstrating its ability to preserve critical visual information under aggressive compression.

\noindent\textbf{Results on LLaVA-NeXT-7B}. Table \ref{tab:llava16_main} presents the corresponding comparison results. SIEVE likewise achieves the best reported average performance with complete results under the 320-token setting, preserving 97.5\% of the Vanilla baseline.
Compared with DART and HoloV, SIEVE improves the average performance by 1.4 and 1.3 percentage points, respectively.
These results demonstrate that SIEVE generalizes effectively from the standard LLaVA-1.5 architecture to the higher-resolution LLaVA-NeXT architecture, which contains substantially more visual tokens.


\noindent\textbf{Results on Qwen2.5-VL.}
Table~\ref{tab:qwen2.5} reports the results on Qwen2.5-VL-7B.
We fix the input resolution to $1008 \times 1008$, corresponding to 1,296 visual tokens per image.
Under token retention ratios of 33.3\%, 22.2\%, and 11.1\%, SIEVE achieves 99.7\%, 98.9\%, and 96.7\% average performance, respectively, consistently outperforming both FastV and HoloV.
Notably, under the most aggressive 11.1\% token budget, SIEVE surpasses FastV and HoloV by 9.2 and 2.3 percentage points, respectively, demonstrating its stronger ability to preserve critical visual information under severe compression.
These results show that SIEVE generalizes effectively beyond the LLaVA family and maintains consistent performance advantages on the Qwen2.5-VL architecture.


\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{8pt}
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{lccccc}
        \toprule
        $\eta \backslash H_{\mathrm{top}}$
        & 8 & 12 & 16 & 24 & 32 \\
        \midrule
        0.65 & 96.15 & 96.35 & 96.29 & 96.42 & 96.26 \\ 
        %0.70 & 96.25 & 96.49 & 96.38 & 96.26 & 96.05 \\ 
        0.75 & 96.17 & \textbf{96.59} & 96.07 & 96.05 & 96.20 \\
        0.85 & 96.25 & 96.48 & 96.15 & 96.16 & 96.29 \\
        %0.90 & 96.31 & 96.34 & 96.20 & 96.34 & 96.25 \\
        0.95 & 96.37 & 96.40 & 96.27 & 96.47 & 96.35 \\
        \bottomrule
    \end{tabular}
    \caption{
        Hyperparameter sensitivity of SIEVE on LLaVA-1.5-7B at
        11.1\% visual-token retention. 
    }
    % Each entry reports the average
    %     percentage relative to the full-token baselines for a selected
    %     combination of energy ratio $\eta$ and image-head top-$k$
    %     value $H_{\mathrm{top}}$. The best result is shown in bold.
    \label{tab:hyper_sensitivity_main}
\end{table}


\subsection{Ablation Study and Analysis}
\paragraph{Hyperparameter Sensitivity.}

We further evaluate the sensitivity of SIEVE to the energy ratio $\eta$ and the number of selected image-attending heads $H_{\mathrm{top}}$, with detailed results provided in Appendix D.

Table~\ref{tab:hyper_sensitivity_main} shows part results. SIEVE achieves the best average retention of 96.59\% with $\eta=0.75$ and $H_{\mathrm{top}}=12$.
Other configurations obtain highly similar results, ranging from 96.05\% to 96.52\%, indicating that SIEVE is robust to hyperparameter choices and does not rely on delicate tuning.


% \begin{table}[t]
% \centering
% \caption{
% Hyperparameter sensitivity of SIEVE on LLaVA-1.5-7B at 11.1\% visual-token retention. Only the average percentage relative to the full-token baseline is reported.
% }
% \label{tab:hyper_sensitivity_main}
% \fontsize{7.6pt}{8.25pt}\selectfont
% \setlength{\tabcolsep}{4.2pt}
% \renewcommand{\arraystretch}{0.90}
% \begin{tabular}{ccc}
% \toprule
% Energy Ratio $\eta$ & $H_{\mathrm{top}}$ & Avg. \%Full \\
% \midrule
% 0.75 & 12 & \textbf{96.59} \\
% 0.98 & 24 & 96.52 \\
% 0.98 & 32 & 96.52 \\
% 0.99 & 16 & 96.51 \\
% 0.98 & 28 & 96.51 \\
% 0.60 & 12 & 96.49 \\
% 0.85 & 12 & 96.48 \\
% 0.95 & 24 & 96.47 \\
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrr}
\toprule
Group & Variant & Avg. \%Full & $\Delta$Avg. \\
\midrule
Full & \textbf{SIEVE full} & \textbf{96.59} & 0.00 \\
\midrule
Score & Attention score only & 96.07 & -0.52 \\
Score & CMR score only & 96.00 & -0.59 \\
Score & (Attention + CMR) score & 96.20 & 0.39 \\
\midrule
Diversity & Top-$K$ selection & 90.13 & -6.46 \\
Diversity & Raw-space diversity & 95.70 & -0.89 \\
\bottomrule
\end{tabular}
\caption{
Component ablation of SIEVE on LLaVA-1.5-7B at 11.1\% visual token retention. Avg. \%Full reports average performance on SQA, TextVQA, POPE, and MME relative to the full-token baseline, while $\Delta$Avg. is measured against full SIEVE. Ablations cover scoring and diversity selection.
}
\label{tab:component_ablation_main}
\end{table}


\paragraph{Component Ablation.}
To assess the contribution of each component, we ablate SIEVE on LLaVA-1.5-7B under 11.1\% visual token retention from two aspects: scoring signals and diversity selection, as shown in Table~\ref{tab:component_ablation_main}.

For scoring, using only the attention score and only the CMR score achieves 96.07\% and 96.00\%, respectively, showing that the geometric residual captured by CMR is itself an effective selection signal rather than an auxiliary term of attention. Combining the two signals multiplicatively gives the full SIEVE result of 96.59\%, outperforming either signal alone. In contrast, additive fusion reaches only 96.20\%, lagging behind multiplicative fusion.

For diversity selection, direct top-$k$ selection drops sharply to 90.13\% ($-6.46$), indicating that selecting tokens solely by the initial scores tends to retain redundant tokens. Raw-space diversity recovers most of the performance to 95.70\% ($-0.89$), but still underperforms full SIEVE, suggesting that enforcing diversity in the residual space is more effective for suppressing redundant visual information.

\paragraph{Effectiveness Analysis of the Fusion Strategy.}
Attention and CMR capture complementary aspects of token importance, namely semantic relevance and geometric residual, respectively. The former focuses on regions directly related to the query, whereas the latter highlights visual regions that cannot be well explained by the text subspace. As shown in Figure~\ref{fig:fusion}, although both respond to informative regions, the overlap between their selected tokens remains consistently low, with a low average overlap ratio across the four benchmarks (see Appendix~E for details). This indicates that the two signals are complementary rather than redundant: relying on either one alone inevitably misses tokens preferred by the other. Consequently, combining the two scores preserves a more complete set of informative visual tokens, leading to better performance than using either attention or CMR alone.

Furthermore, multiplicative fusion is better aligned with this objective than additive fusion. Additive fusion is sensitive to differences in score magnitude, allowing one signal to dominate the final ranking. In contrast, multiplicative fusion favors tokens that simultaneously exhibit semantic relevance and substantial residual information, while naturally suppressing background or noisy tokens that receive an abnormally high score from only one signal. As a result, additive fusion achieves only 96.20\%, lower than the 96.59\% obtained by multiplicative fusion.


\begin{table}
\centering
\small
\setlength{\tabcolsep}{3.2pt}

\begin{tabular}{ll|c|c|c|c}
\toprule
\textbf{Model} &
\textbf{Method} &
\begin{tabular}[c]{@{}c@{}}\textbf{Total}\\\textbf{Time}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Prefill}\\\textbf{Time}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{KV Cache}\\\textbf{(MB)}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{POPE}\\\textbf{F1}\end{tabular} \\
\midrule

\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}LLaVA-\\NeXT-7B\end{tabular}}
& Full       & 46:11 & 37:21 & 1156 & 86.5 \\
& Random     & 15:33 & 7:20  & 192  & 79.1 \\
& SparseVLM  & 35:55 & 26:57 & 200  & 82.4 \\

& SIEVE       & 18:32 & 10:20 & 192  & 85.7 \\
\midrule

\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}LLaVA-\\1.5-7B\end{tabular}}
& Full       & 16:39 & 9:55 & 319 & 85.9 \\
& Random     & 10:49 & 4:10 & 63  & 75.8 \\
& SparseVLM  & 12:58 & 6:18 & 66  & 77.5 \\

& SIEVE       & 11:36 & 4:56 & 63  & 83.4 \\

\bottomrule
\end{tabular}%
\caption{
Efficiency comparison on POPE for LLaVA-NeXT-7B and LLaVA-1.5-7B.
All token reduction methods retain 11.1\% visual tokens.
}
\label{tab:efficiency_comparison}
\end{table}


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{Images/stop_and_four_people_layer16_top115.pdf}
    \caption{
Different selection between attention and CMR.
    }
    \label{fig:fusion}
\end{figure}





\paragraph{Efficiency Analysis.}
SIEVE achieves a strong trade-off between efficiency and performance. As shown in Table~\ref{tab:efficiency_comparison}, compared with the full model, SIEVE achieves 2.49$\times$/1.44$\times$ total runtime speedups and 3.62$\times$/2.01$\times$ prefill speedups on LLaVA-NeXT/LLaVA-1.5, while reducing the KV cache from 1156MB/319MB to 192MB/63MB.
Even compared with Random pruning, which approximates an ideal fast baseline, SIEVE remains close in runtime, with only 19\%/7\% additional total time, while improving POPE F1 by 6.6/7.6 points.
Compared with SparseVLM, SIEVE is faster on both models in total runtime and prefill time while maintaining higher accuracy.
%Overall, SIEVE reduces inference latency and KV cache overhead while preserving strong performance, resulting in a better balance between efficiency and performance.






==> Sections_Introduction.tex <==
\section{Introduction}\label{Introduction}

Vision Language Models (VLMs) have achieved remarkable progress in multimodal tasks such as visual question answering, image captioning, and document understanding. Representative models, including LLaVA~\cite{liu2023llava}, InternVL~\cite{chen2024internvl}, and Qwen-VL~\cite{bai2023qwen}, typically encode images into numerous visual tokens and feed them into large language models together with text tokens for joint reasoning. However, the increasing number of visual tokens substantially raises self-attention computation, leading to higher inference latency and computational cost. This overhead is further amplified in high-resolution images, multi-image inputs, and video understanding. Therefore, compressing visual tokens while preserving model capability is crucial for efficient VLM inference.

Existing visual token compression methods mainly select tokens based on current layer attention~\cite{chen2024FastV,zhang2025sparsevlm} or feature similarity~\cite{bolya2023tome,wen2025dart}: the former characterizes the relevance between visual tokens and the current textual context, whereas the latter measures the redundancy among visual tokens. Although these signals provide useful criteria, they only characterize the local state at a single layer and lack a holistic view of the entire multimodal reasoning process. To this end, we revisit the inference process of VLMs, rather than staying at the local state of a single layer, and observe that as LLM layers deepen, text tokens continuously aggregate visual information through self-attention, progressively integrating part of the visual content into the textual representations. 

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth,height=0.25\textwidth,keepaspectratio]{Images/absorption_3d_cmr_closer_layers_1_16_32_font_larger_150.pdf}
\caption{3D visualization of visual tokens relative to the text subspace. Text tokens are centered and projected by PCA to obtain the first two principal directions, denoted as Text PC1 and Text PC2. Visual tokens are centered using the same text mean and projected onto these directions to obtain planar coordinates, while height and color indicate their CMR.
More results are provided in Appendix~A.}

 %Text tokens are centered and projected by PCA to obtain the first two principal directions, denoted as Text PC1 and Text PC2. Visual tokens are centered using the same text mean and projected onto these directions to obtain planar coordinates, while height and color indicate their CMR.
\label{fig:cmr_3d_visualization}
\end{figure}

To quantify this phenomenon, we propose Cross Modal Absorption (CMA) from a geometric representation perspective, which measures at the layer level the overall extent to which visual token representations are absorbed by text, i.e., explainable by the text subspace. CMA characterizes the absorption trend at the layer level, whereas compression must operate on individual tokens. We therefore refine this perspective to the token level and propose Cross Modal Residual (CMR). Specifically, each visual token is projected onto the text subspace with Tikhonov regularization, and the reconstruction residual is used to quantify the visual information unexplained by text. A larger residual indicates that the token carries more unique visual information and thus has a higher retention necessity. This projection can be efficiently solved in closed form via regularized least squares, introducing only minor additional overhead. As shown in Figure~\ref{fig:cmr_3d_visualization}, visual token representations gradually move closer to the text subspace as layer depth increases, indicating that visual information does not always remain independent, but is progressively integrated into the text representation space.

% Across multiple benchmarks, CMA increases monotonically with layer depth, showing that more visual tokens in deeper layers can be approximately explained by the text subspace, and thus the necessity of retaining them in full decreases accordingly. 




Building on the above analysis, we propose \textbf{SIEVE}, a training-free visual token compression method that selects tokens from three complementary perspectives: CMR for visual distinctiveness and text-to-visual attention relevance for task relevance, so that retained tokens both carry unique visual information and align with the current textual context, together with diversity selection in the residual space to remove redundancy. Unlike de-duplication in the original feature space, the residual space has already removed the components explainable by text, so its directions more directly reflect the unique visual information of each token, enabling more precise identification of genuinely complementary tokens. SIEVE is training-free and plug-and-play, making it directly applicable to existing VLMs.

In summary, our contributions are threefold:
\begin{itemize}

% \item \textbf{Analytical.} To our knowledge, the necessity of retaining visual tokens has not been examined from the perspective of cross modal reasoning dynamics. We propose CMA to quantify, at the layer level, how much visual information is absorbed by text, revealing that visual tokens become progressively more explainable by the text subspace as depth increases, and CMR to measure, at the token level, the residual visual information unexplained by text.

\item We propose a novel pruning guidance criterion named CMR. Unlike mainstream token pruning approaches guided by token similarity, we revisit the model inference process and identify the phenomenon where visual information is gradually assimilated by textual information. We then quantify this process to develop CMR.

% To our knowledge, the necessity of retaining visual tokens has not been examined from the perspective of cross modal reasoning dynamics. We propose CMA to quantify, at the layer level, how much visual information is absorbed by text, revealing that visual tokens become progressively more explainable by the text subspace as depth increases, and CMR to measure, at the token level, the residual visual information unexplained by text.

\item We propose SIEVE, a training-free visual token compression method that jointly selects tokens using CMR, attention relevance, and residual-space diversity selection, balancing visual distinctiveness, task relevance, and complementarity. 
%, with CMR efficiently solvable in closed form.

\item Extensive experiments across three VLM architectures and eight benchmarks demonstrate that the proposed method significantly reduces computational overhead and memory, delivering practical inference acceleration.

%\textbf{Experimental.} SIEVE delivers strong performance--efficiency trade-offs across VLM architectures and token budgets. On LLaVA-NeXT-7B, retaining only 11.1\% of visual tokens preserves 97.5\% of the original average performance, while achieving 3.62$\times$ prefill speedup, 2.49$\times$ end-to-end speedup, and 6.02$\times$ KV-cache reduction.


\end{itemize}

==> Sections_Method.tex <==

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth]{Images/overall.pdf}
%     \caption{
%     Overview of SIEVE. SIEVE measures each visual token’s residual information with respect to the text subspace via CMR, combines it with attention relevance, and performs residual-space diversity selection to retain informative and non-redundant visual tokens for the compressed input sequence.
%     }
%     \label{fig:overall}
% \end{figure*}
\section{Method}\label{Method}
Since CMA operates at the layer level while compression acts on individual tokens, we refine it to the token level and propose \textbf{SIEVE}, a training-free visual token compression method that selects tokens from three complementary perspectives: CMR, text-attention relevance, and residual-space diversity, as shown in Figure~\ref{fig:overall}

\subsection{Constructing the CMR Score}

SIEVE first constructs a Cross Modal Residual (CMR) score to measure the residual information in each visual token that cannot be explained by the text subspace: a lower score means higher redundancy, a higher one more distinctive visual information. At the $l$-th pruning layer, let $T \in \mathbb{R}^{N_t \times D}$ and $V \in \mathbb{R}^{N_v \times D}$ denote the text- and visual-token representation matrices, where $D$ is the hidden dimension. SIEVE first centers both modalities using the mean text representation:
\begin{equation}
\bar{t}
=
\frac{1}{N_t}
\sum_{j=1}^{N_t}
T_j,
\quad
T_c
=
T-\bar{t},
\quad
V_c
=
V-\bar{t}.
\end{equation}
Here $\bar{t}$ is the mean text representation, and $T_c$, $V_c$ are the centered text and visual matrices. Using the text center as reference reduces the background components shared between the two modalities and highlights each visual token's unique deviation from the text subspace.

For the $i$-th centered visual token $v_{c,i}$, SIEVE reconstructs it as a linear combination of text tokens, using a Tikhonov-regularized least-squares formulation for stability:
\begin{equation}
b_i
=
\arg\min_{b_i \in \mathbb{R}^{1 \times N_t}}
\left\|
v_{c,i}
-
b_iT_c
\right\|_2^2
+
\lambda
\left\|
b_i
\right\|_2^2 .
\end{equation}
Here $b_i$ are the combination coefficients of $v_{c,i}$ over text tokens and $\lambda$ is the regularization coefficient. The first term measures the reconstruction error from the text subspace, while the second constrains the coefficient magnitude to prevent unstable solutions caused by low-energy directions.

To adaptively determine $\lambda$, SIEVE constructs the text Gram matrix:
\begin{equation}
G
=
T_cT_c^\top .
\end{equation}
Here $G \in \mathbb{R}^{N_t \times N_t}$ characterizes the energy distribution of the text subspace, providing the basis for setting $\lambda$. Sorting its eigenvalues in descending order as $\sigma_1^2 \geq \cdots \geq \sigma_{N_t}^2$ and given an energy ratio threshold $\eta$, SIEVE selects the smallest $k$ satisfying
\begin{equation}
\sum_{j=1}^{k}
\sigma_j^2
\geq
\eta
\sum_{j=1}^{N_t}
\sigma_j^2 .
\end{equation}
Here $\eta$ is the energy proportion to be covered and $k$ is the number of dominant directions needed to reach it, delimiting the effective dimensionality of the text subspace. The regularization coefficient is then set as
\begin{equation}
\lambda
=
\sigma_k^2
+
\epsilon ,
\end{equation}
where $\epsilon$ is a small constant for numerical stability. Setting $\lambda$ to the $k$-th eigenvalue lets the dominant directions contribute fully to reconstruction while suppressing instability from low-energy directions. This yields the closed-form solution and the reconstruction:
\begin{equation}
b_i
=
v_{c,i}T_c^\top
\left(
G+\lambda I
\right)^{-1},
\qquad
\hat{v}_{c,i}
=
b_iT_c .
\end{equation}
Here $I$ is the identity matrix and $\hat{v}_{c,i}$ is the visual token reconstructed from the text subspace; the closed-form solution avoids iterative optimization and adds only negligible overhead. Finally, SIEVE defines the CMR score as the ratio between the reconstruction residual and the original centered representation:
\begin{equation}
\mathrm{CMR}_i
=
\frac{
\left\|
v_{c,i}
-
\hat{v}_{c,i}
\right\|_2
}{
\left\|
v_{c,i}
\right\|_2
}.
\end{equation}
Normalizing the residual by the original norm removes the effect of differing token magnitudes. A lower $\mathrm{CMR}_i$ means the token is well reconstructed by the text subspace and can be preferentially pruned, while a higher $\mathrm{CMR}_i$ means it preserves a larger text-unexplained residual and should be preferentially retained.
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{7pt}

\begin{tabular}{l|l|cccccccc|c}
\toprule
\textbf{Methods} & \textbf{Venue}
& \textbf{GQA} & \textbf{MMB} & \textbf{MMB-cn} & \textbf{MME}
& \textbf{POPE} & \textbf{SQA} & \textbf{VQAv2} & \textbf{TextVQA}
& \textbf{Average} \\
\midrule


\textbf{LLaVA-1.5-7B}
&
& \multicolumn{8}{c|}{\textbf{Upper Bound, 576 Tokens}}
& \\
Vanilla & --
& 61.9 & 64.7 & 58.1 & 1862 & 85.9 & 69.5 & 78.5 & 58.2
& \textbf{100\%} \\

\midrule

\textbf{LLaVA-1.5-7B}
&
& \multicolumn{8}{c|}{\textbf{Retain 192 Tokens (33.3\%)}}
& \\
FastV & ECCV'24
& 52.7 & 61.2 & 57.0 & 1612 & 64.8 & 67.3 & 67.1 & 52.5
& 89.0\% \\
% PDrop & CVPR'25
% & 57.1 & 63.2 & 56.8 & 1766 & 82.3 & 68.8 & 75.1 & 56.1
% & 96.2\% \\
SparseVLM & ICML'25
& 59.5 & 64.1 & 53.7 & 1787 & 85.3 & 68.7 & 75.6 & 57.8
& 97.2\% \\
DART & EMNLP'25
& 60.0 & 63.6 & 57.0 & 1856 & 82.8 & 69.8 & 76.7 & 57.4
& 98.3\% \\
VisionZip & CVPR'25
& 59.3 & 63.0 & 57.3 & 1782 & 85.3 & 68.9 & 76.8 & 57.3
& 97.8\% \\
HoloV & NeurIPS'25
& 59.0 & 65.4 & 58.0 & 1820 & 85.6 & 69.8 & 76.7 & 57.4
& 98.7\% \\
SCOPE & NeurIPS'25
& 60.1 & 63.6 & 56.8 & 1804 & 86.4 & 68.8 & 77.2 & 57.7
& 98.3\% \\
SpecFlow & ICML'26
& 58.3 & 65.8 & 56.1 & 1827 & 85.8 & 69.7 & 76.4 & 57.9
& 98.4\% \\

\textbf{SIEVE}  & \textbf{Ours}
& 60.6 & 64.6 & 58.4 & 1820 & 85.5 & 68.9 & 77.8 & 57.8
& \textbf{99.1\%} \\

\midrule

\textbf{LLaVA-1.5-7B}
&
& \multicolumn{8}{c|}{\textbf{Retain 128 Tokens (22.2\%)}}
& \\
FastV & ECCV'24
& 49.6 & 56.1 & 56.4 & 1490 & 59.6 & 60.2 & 61.8 & 50.6
& 83.2\% \\
% PDrop & CVPR'25
% & 56.0 & 61.1 & 56.6 & 1644 & 82.3 & 68.3 & 72.9 & 55.1
% & 94.0\% \\
SparseVLM & ICML'25
& 58.4 & 64.5 & 51.1 & 1746 & 85.0 & 68.6 & 73.8 & 56.7
& 95.6\% \\
DART & EMNLP'25
& 58.7 & 63.2 & 57.5 & 1840 & 80.1 & 69.1 & 75.9 & 56.4
& 97.0\% \\
VisionZip & CVPR'25
& 57.6 & 62.0 & 56.7 & 1761.7 & 83.2 & 68.9 & 75.6 & 56.8
& 96.4\% \\
HoloV & NeurIPS'25
& 57.7 & 63.9 & 56.5 & 1802 & 84.0 & 69.8 & 75.5 & 56.8
& 97.2\% \\
SCOPE & NeurIPS'25
& 59.7 & 62.5 & 56.9 & 1776 & 86.1 & 68.4 & 76.5 & 57.2
& 97.5\% \\
SpecFlow & ICML'26
& 57.6 & 64.3 & 55.9 & 1794 & 84.9 & 69.9 & 75.3 & 56.8
& 97.2\% \\

\textbf{SIEVE}  & \textbf{Ours}
& 59.8 & 64.0 & 57.0 & 1815 & 85.8 & 68.8 & 77.1 & 57.6
& \textbf{98.7\%} \\

\midrule

\textbf{LLaVA-1.5-7B}
&
& \multicolumn{8}{c|}{\textbf{Retain 64 Tokens (11.1\%)}}
& \\
FastV & ECCV'24
& 46.1 & 48.0 & 52.7 & 1256 & 48.0 & 51.1 & 55.0 & 47.8
& 74.0\% \\
% PDrop & CVPR'25
% & 41.9 & 33.3 & 50.5 & 1092 & 55.9 & 68.6 & 69.2 & 45.9
% & 74.4\% \\
SparseVLM & ICML'25
& 53.8 & 60.1 & 52.7 & 1589 & 77.5 & 69.8 & 68.2 & 53.4
& 90.6\% \\
DART & EMNLP'25
& 55.9 & 60.6 & 53.2 & 1765 & 73.9 & 69.8 & 72.4 & 54.4
& 92.8\% \\
VisionZip & CVPR'25
& 55.1 & 60.1 & 55.4 & 1690 & 77.0 & 69.0 & 72.4 & 55.5
& 93.0\% \\
HoloV & NeurIPS'25
& 55.3 & 63.3 & 55.1 & 1715 & 80.3 & 69.5 & 72.8 & 55.4
& 94.4\% \\
SCOPE & NeurIPS'25
& 58.3 & 61.7 & 54.4 & 1698 & 83.9 & 68.6 & 75.3 & 56.6
& 95.4\% \\
SpecFlow & ICML'26
& 55.3 & 63.7 & 54.3 & 1713 & 80.5 & 69.7 & 73.7 & 54.9
& 94.4\% \\

\textbf{SIEVE}  & \textbf{Ours}
& 58.0 & 62.2 & 55.2 & 1740 & 83.5 & 69.0 & 75.2 & 56.5
& \textbf{96.0\%} \\
\bottomrule
\end{tabular}
\caption{Performance comparison of different token reduction methods on LLaVA-1.5-7B.}
\label{tab:llava15_main}
\end{table*}
\subsection{Attention Signal Construction}

CMR measures the unique information in a visual token that cannot be explained by the text subspace, but geometric uniqueness does not necessarily indicate relevance to the current text context. Therefore, SIEVE further introduces an attention signal to determine whether each visual token is actually attended to by the text tokens. For the $i$-th visual token, its text relevance score is defined as
\begin{equation}
a_i
=
\sum_{h \in \mathcal{H}_{\mathrm{top}}}
\sum_{t \in \mathcal{T}}
\alpha_{t,i}^{h}.
\end{equation}
Here, $\mathcal{T}$ denotes the set of text tokens, and $\alpha_{t,i}^{h}$ denotes the attention weight from text token $t$ to visual token $i$ in the $h$-th attention head. To reduce the influence of noisy heads, SIEVE keeps only the top $\rho_h$ proportion of heads with the largest attention mass on the visual region, denoted as $\mathcal{H}_{\mathrm{top}}$. A larger $a_i$ indicates stronger relevance to the current textual context. 

SIEVE does not need to explicitly store the full attention matrix. Following the dual-flash attention strategy in SparseVLM~\cite{zhang2025sparsevlm}, SIEVE can compute the required attention signal while remaining compatible with FlashAttention, with details provided in Appendix C.

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5.2pt}

\begin{tabular}{l|l|cccccccc|c}
\toprule
\textbf{Method} & \textbf{Venue}
& \textbf{GQA} & \textbf{MMBench} & \textbf{MMBench-cn} & \textbf{MME}
& \textbf{POPE} & \textbf{SQA} & \textbf{VQAv2} & \textbf{TextVQA}
& \textbf{Avg} \\
\midrule

\textbf{LLaVA-NeXT-7B}
&
& \multicolumn{8}{c|}{\textbf{Upper Bound, 2880 Tokens}}
& \\
Vanilla & --
& 64.2 & 67.4 & 60.6 & 1851 & 86.5 & 70.1 & 81.8 & 61.4
& 100\% \\
\midrule

\textbf{LLaVA-NeXT-7B}
&
& \multicolumn{8}{c|}{\textbf{Retain 320 Tokens}}
& \\
FastV & ECCV'24
& 55.9 & 61.6 & 51.9 & 1661 & 71.7 & 62.8 & 71.9 & 55.7
& 88.1\% \\
SparseVLM & ICML'25
& 56.1 & 60.6 & 54.5 & 1533 & 82.4 & 66.1 & 71.5 & 58.4
& 90.3\% \\
VisionZip & CVPR'25
& 59.3 & 63.1 & 55.6 & 1702 & 82.1 & 67.3 & 76.2 & 58.9
& 93.7\% \\
DART & EMNLP'25
& 61.7 & 65.3 & 58.2 & 1710 & 84.1 & 68.4 & 79.1 & 58.7
& 96.1\% \\
HoloV & NeurIPS'25
& 61.7 & 65.3 & 57.5 & 1738 & 83.9 & 68.9 & 79.5 & 58.7
& 96.2\% \\
SpecFlow & ICML'26
& 62.5 & 66.7 & 56.8 & 1707 & 85.0 & 68.6 & 80.1 & 59.5
& 96.6\% \\

\textbf{SIEVE} & \textbf{Ours}
& 60.9 & 66.5 & 59.6 & 1819 & 85.7 & 68.3 & 78.7 & 59.6
& \textbf{97.5\%} \\
\bottomrule
\end{tabular}%
\caption{Performance comparison of different token reduction methods on LLaVA-NeXT-7B.}
\label{tab:llava16_main}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{7.1pt}

\begin{tabular}{l|l|ccccccc|c}
\toprule
\textbf{Method} & \textbf{Venue}
& \textbf{MMBench} & \textbf{MME} & \textbf{POPE} & \textbf{SQA}
& \textbf{MMBench-cn} & \textbf{GQA} & \textbf{TextVQA} & \textbf{Avg} \\
\midrule

\textbf{Qwen2.5-VL-7B} &
& \multicolumn{7}{c|}{\textbf{Upper Bound, 1296 Tokens}} & \\
Vanilla & --
& 83.4 & 2295 & 87.1 & 88.7 & 81.4 & 61.0 & 77.2 & 100.0\% \\
\midrule

\textbf{Qwen2.5-VL-7B} &
& \multicolumn{7}{c|}{\textbf{Retain 33.3\% Tokens}} & \\
FastV & ECCV'24
& 79.5 & 2306 & 86.9 & 85.6 & 77.9 & 59.5 & 75.0 & 97.5\% \\
HoloV & NeurIPS'25
& 81.2 & 2288.9 & 86.1 & 88.7 & 80.0 & 60.2 & 74.4 & 98.5\% \\

\textbf{SIEVE}  & \textbf{Ours}
& 82.5 & 2319 & 88.0 & 88.2 & 81.3 & 60.8 & 75.8 & \textbf{99.7\%} \\
\midrule

\textbf{Qwen2.5-VL-7B} &
& \multicolumn{7}{c|}{\textbf{Retain 22.2\% Tokens}} & \\
FastV & ECCV'24
& 76.5 & 2243 & 85.1 & 84.8 & 75.2 & 57.8 & 73.5 & 95.0\% \\
HoloV & NeurIPS'25
& 80.5 & 2268.8 & 85.2 & 88.2 & 79.6 & 59.5 & 71.7 & 97.2\% \\

\textbf{SIEVE}  & \textbf{Ours}
& 81.6 & 2313 & 87.3 & 87.5 & 80.2 & 60.3 & 75.1 & \textbf{98.9\%} \\
\midrule

\textbf{Qwen2.5-VL-7B} &
& \multicolumn{7}{c|}{\textbf{Retain 11.1\% Tokens}} & \\
FastV & ECCV'24
& 71.2 & 2061 & 78.6 & 80.6 & 68.2 & 52.4 & 67.0 & 87.5\% \\
HoloV & NeurIPS'25
& 78.2 & 2246.5 & 83.7 & 87.6 & 77.1 & 57.5 & 65.7 & 94.4\% \\

\textbf{SIEVE}  & \textbf{Ours}
& 80.0 & 2273 & 86.0 & 86.6 & 77.6 & 58.9 & 72.5 & \textbf{96.7\%} \\
\bottomrule
\end{tabular}%
\caption{Performance comparison of different token reduction methods on Qwen2.5-VL-7B.}
\label{tab:qwen2.5}
\end{table*}

\subsection{Guided Scores}

SIEVE initializes each token's integrated score as
\begin{equation}
\mathrm{Score}_i = a_i^2 \, \mathrm{CMR}_i^2,
\end{equation}
where $a_i$ is the text-relevance (attention) score and $\mathrm{CMR}_i$ is the residual ratio unexplained by the text subspace; the product keeps attention from overlooking residual information and CMR from ignoring textual relevance.

\subsection{Residual-Space Diversity Selection}

Given the guided scores defined above, SIEVE aims to retain visual tokens that are both individually informative and mutually complementary. To this end, it performs residual-space diversity selection in two stages: it first measures the redundancy between visual tokens in the residual space, and then greedily selects tokens while progressively suppressing redundant candidates.

\begin{enumerate}
    \item \textbf{Residual Similarity Measurement.}
    Selecting the top-$K$ tokens by integrated score alone may retain tokens with similar residual directions, causing visual redundancy. To avoid this, SIEVE measures token redundancy in the \emph{residual space} rather than the original space: the residual removes the large shared component that otherwise dominates the cosine similarity, so comparisons reflect each token's genuinely complementary information. 
    For the $i$-th centered visual token $v_{c,i}$ with text-subspace reconstruction $\hat{v}_{c,i}$, the residual is
    \begin{equation}
    r_i = v_{c,i} - \hat{v}_{c,i},
    \end{equation}
    i.e., the part the text subspace cannot reconstruct. Redundancy between two tokens is measured by the squared cosine similarity of their residuals,
    \begin{equation}
    g_{ij}
    =
    \left(
    \frac{r_i^\top r_j}
    {\left\|r_i\right\|_2\left\|r_j\right\|_2}
    \right)^2
    \in [0,1],
    \end{equation}
    where a larger $g_{ij}$ means more similar residual directions and thus higher redundancy.

    \item \textbf{Diversity-Aware Greedy Selection.}
    Based on the guided scores and residual similarities, SIEVE iteratively selects informative and non-redundant visual tokens. At each step, it selects
    \begin{equation}
    i^\ast
    =
    \arg\max_{i \notin \mathcal{S}}
    \mathrm{Score}_i,
    \end{equation}
    with $\mathcal{S}$ the set of selected tokens, and then discounts the remaining candidates by their residual similarity to $i^\ast$:
    \begin{equation}
    \mathrm{Score}_j
    \leftarrow
    \mathrm{Score}_j(1-g_{i^\ast j}),
    \quad j \notin \mathcal{S}.
    \end{equation}
    Since $g_{i^\ast j}\in[0,1]$ is a dimensionless quantity normalized by the residual magnitudes, the factor $1-g_{i^\ast j}$ is a scaling coefficient in $[0,1]$ that attenuates $\mathrm{Score}_j$ proportionally without altering its dimension. Candidates whose residual directions align with the selected token are thereby progressively suppressed, and the process continues until the budget $K$ is reached.
\end{enumerate}

% \subsection{Residual-Space Diversity Selection}

% \subsubsection{Residual Similarity Measurement}

% Selecting the top-$K$ tokens by integrated score alone may retain tokens with similar residual directions, causing visual redundancy. To avoid this, SIEVE performs greedy diversity selection in the \emph{residual space} rather than the original feature space: the residual removes the large shared component that otherwise dominates the cosine similarity, so comparisons reflect each token's genuinely complementary information.

% For the $i$-th centered visual token $v_{c,i}$ with text-subspace reconstruction $\hat{v}_{c,i}$, the residual is
% \begin{equation}
% r_i = v_{c,i} - \hat{v}_{c,i},
% \end{equation}
% i.e., the part the text subspace cannot reconstruct. Redundancy between two tokens is measured by the squared cosine similarity of their residuals,
% \begin{equation}
% g_{ij} = \left( \frac{r_i^\top r_j}{\left\|r_i\right\|_2 \left\|r_j\right\|_2} \right)^2 \in [0,1],
% \end{equation}
% where a larger $g_{ij}$ means more similar residual directions and thus higher redundancy.

% \subsubsection{Diversity-Aware Greedy Selection}

% At each step SIEVE selects
% \begin{equation}
% i^\ast = \arg\max_{i \notin \mathcal{S}} \mathrm{Score}_i ,
% \end{equation}
% with $\mathcal{S}$ the set of selected tokens, and then discounts the remaining candidates by their residual similarity to $i^\ast$:
% \begin{equation}
% \mathrm{Score}_j \leftarrow \mathrm{Score}_j \, (1 - g_{i^\ast j}), \quad j \notin \mathcal{S}.
% \end{equation}
% Since $g_{i^\ast j}\in[0,1]$ is a dimensionless quantity normalized by the residual magnitudes, the factor $1-g_{i^\ast j}$ is a scaling coefficient in $[0,1]$ that attenuates $\mathrm{Score}_j$ proportionally without altering its dimension. Candidates whose residual directions align with the selected token are thereby progressively suppressed, and the process continues until the budget $K$ is reached.
% \subsection{Attention Signal Construction}

% CMR measures the unique information in a visual token that cannot be explained by the text subspace, but geometric uniqueness does not necessarily indicate relevance to the current text context. Therefore, SIEVE further introduces an attention signal to determine whether each visual token is actually attended to by the text tokens. For the $i$-th visual token, its text relevance score is defined as
% \begin{equation}
% a_i
% =
% \sum_{h \in \mathcal{H}_{\mathrm{top}}}
% \sum_{t \in \mathcal{T}}
% \alpha_{t,i}^{h}.
% \end{equation}
% Here, $\mathcal{T}$ denotes the set of text tokens, and $\alpha_{t,i}^{h}$ denotes the attention weight from text token $t$ to visual token $i$ in the $h$-th attention head. To reduce the influence of noisy heads, SIEVE keeps only the top $\rho_h$ proportion of heads with the largest attention mass on the visual region, denoted as $\mathcal{H}_{\mathrm{top}}$. A larger $a_i$ indicates stronger relevance to the current textual context. 

% SIEVE does not need to explicitly store the full attention matrix. Following the dual-flash attention strategy in SparseVLM~\cite{zhang2025sparsevlm}, SIEVE can compute the required attention signal while remaining compatible with FlashAttention, with details provided in Appendix C.
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{2pt}

% \begin{tabular}{l|l|cccccccc|c}
% \toprule
% \textbf{Method} & \textbf{Venue}
% & \textbf{GQA} & \textbf{MMBench} & \textbf{MMBench-cn} & \textbf{MME}
% & \textbf{POPE} & \textbf{SQA} & \textbf{VQAv2} & \textbf{TextVQA}
% & \textbf{Avg} \\
% \midrule


% \textbf{LLaVA-NeXT-7B}
% &
% & \multicolumn{8}{c|}{\textbf{Upper Bound, 2880 Tokens}}
% & \\
% Vanilla & --
% & 64.2 & 67.4 & 60.6 & 1851 & 86.5 & 70.1 & 81.8 & 61.4
% & 100\% \\
% \midrule


% \textbf{LLaVA-NeXT-7B}
% &
% & \multicolumn{8}{c|}{\textbf{Retain 320 Tokens}}
% & \\
% FastV & ECCV'24
% & 55.9 & 61.6 & 51.9 & 1661 & 71.7 & 62.8 & 71.9 & 55.7
% & 88.1\% \\
% SparseVLM & ICML'25
% & 56.1 & 60.6 & 54.5 & 1533 & 82.4 & 66.1 & 71.5 & 58.4
% & 90.3\% \\
% VisionZip & CVPR'25
% & 59.3 & 63.1 & 55.6 & 1702 & 82.1 & 67.3 & 76.2 & 58.9
% & 93.7\% \\
% DART & EMNLP'25
% & 61.7 & 65.3 & 58.2 & 1710 & 84.1 & 68.4 & 79.1 & 58.7
% & 96.1\% \\
% HoloV & NeurIPS'25
% & 61.7 & 65.3 & 57.5 & 1738 & 83.9 & 68.9 & 79.5 & 58.7
% & 96.2\% \\
% SpecFlow & ICML'26
% & 62.5 & 66.7 & 56.8 & 1707 & 85.0 & 68.6 & 80.1 & 59.5
% & 96.6\% \\

% \textbf{SIEVE} & \textbf{Ours}
% & 60.9 & 66.5 & 59.6 & 1819 & 85.7 & 68.3 & 78.7 & 59.6
% & \textbf{97.5\%} \\
% \bottomrule
% \end{tabular}%
% \caption{Performance comparison of different token reduction methods on LLaVA-NeXT-7B.}
% \label{tab:llava16_main}
% \end{table*}
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{2pt}

% \begin{tabular}{l|l|ccccccc|c}
% \toprule
% \textbf{Method} & \textbf{Venue}
% & \textbf{MMBench} & \textbf{MME} & \textbf{POPE} & \textbf{SQA}
% & \textbf{MMBench-cn} & \textbf{GQA} & \textbf{TextVQA} & \textbf{Avg} \\
% \midrule


% \textbf{Qwen2.5-VL-7B} &
% & \multicolumn{7}{c|}{\textbf{Upper Bound, 1296 Tokens}} & \\
% Vanilla & --
% & 83.4 & 2295 & 87.1 & 88.7 & 81.4 & 61.0 & 77.2 & 100.0\% \\
% \midrule


% \textbf{Qwen2.5-VL-7B} &
% & \multicolumn{7}{c|}{\textbf{Retain 33.3\% Tokens}} & \\
% FastV & ECCV'24
% & 79.5 & 2306 & 86.9 & 85.6 & 77.9 & 59.5 & 75.0 & 97.5\% \\
% HoloV & NeurIPS'25
% & 81.2 & 2288.9 & 86.1 & 88.7 & 80.0 & 60.2 & 74.4 & 98.5\% \\

% \textbf{SIEVE}  & \textbf{Ours}
% & 82.5 & 2319 & 88.0 & 88.2 & 81.3 & 60.8 & 75.8 & \textbf{99.7\%} \\
% \midrule


% \textbf{Qwen2.5-VL-7B} &
% & \multicolumn{7}{c|}{\textbf{Retain 22.2\% Tokens}} & \\
% FastV & ECCV'24
% & 76.5 & 2243 & 85.1 & 84.8 & 75.2 & 57.8 & 73.5 & 95.0\% \\
% HoloV & NeurIPS'25
% & 80.5 & 2268.8 & 85.2 & 88.2 & 79.6 & 59.5 & 71.7 & 97.2\% \\

% \textbf{SIEVE}  & \textbf{Ours}
% & 81.6 & 2313 & 87.3 & 87.5 & 80.2 & 60.3 & 75.1 & \textbf{98.9\%} \\
% \midrule


% \textbf{Qwen2.5-VL-7B} &
% & \multicolumn{7}{c|}{\textbf{Retain 11.1\% Tokens}} & \\
% FastV & ECCV'24
% & 71.2 & 2061 & 78.6 & 80.6 & 68.2 & 52.4 & 67.0 & 87.5\% \\
% HoloV & NeurIPS'25
% & 78.2 & 2246.5 & 83.7 & 87.6 & 77.1 & 57.5 & 65.7 & 94.4\% \\

% \textbf{SIEVE}  & \textbf{Ours}
% & 80.0 & 2273 & 86.0 & 86.6 & 77.6 & 58.9 & 72.5 & \textbf{96.7\%} \\
% \bottomrule
% \end{tabular}%
% \caption{Performance comparison of different token reduction methods on Qwen2.5-VL-7B.}
% \label{tab:qwen2.5}
% \end{table*}
% \subsection{Residual Space Diversity Selection}
% Selecting the top-$K$ tokens by integrated score alone may retain tokens with similar residual directions, causing visual redundancy. To avoid this, SIEVE performs greedy diversity selection in the \emph{residual space} rather than the original feature space: the residual removes the large shared component that otherwise dominates the cosine similarity, so comparisons reflect each token's genuinely complementary information.

% For the $i$-th centered visual token $v_{c,i}$ with text-subspace reconstruction $\hat{v}_{c,i}$, the residual is
% \begin{equation}
% r_i = v_{c,i} - \hat{v}_{c,i},
% \end{equation}
% i.e., the part the text subspace cannot reconstruct. Redundancy between two tokens is measured by the squared cosine similarity of their residuals,
% \begin{equation}
% g_{ij} = \left( \frac{r_i^\top r_j}{\left\|r_i\right\|_2 \left\|r_j\right\|_2} \right)^2 \in [0,1],
% \end{equation}
% where a larger $g_{ij}$ means more similar residual directions and thus higher redundancy.

% SIEVE initializes each token's integrated score as
% \begin{equation}
% \mathrm{Score}_i = a_i^2 \, \mathrm{CMR}_i^2,
% \end{equation}
% where $a_i$ is the text-relevance (attention) score and $\mathrm{CMR}_i$ is the residual ratio unexplained by the text subspace; the product keeps attention from overlooking residual information and CMR from ignoring textual relevance. At each step SIEVE selects
% \begin{equation}
% i^\ast = \arg\max_{i \notin \mathcal{S}} \mathrm{Score}_i ,
% \end{equation}
% with $\mathcal{S}$ the set of selected tokens, and then discounts the remaining candidates by their residual similarity to $i^\ast$:
% \begin{equation}
% \mathrm{Score}_j \leftarrow \mathrm{Score}_j \, (1 - g_{i^\ast j}), \quad j \notin \mathcal{S}.
% \end{equation}
% Since $g_{i^\ast j}\in[0,1]$ is a dimensionless quantity normalized by the residual magnitudes, the factor $1-g_{i^\ast j}$ is a scaling coefficient in $[0,1]$ that attenuates $\mathrm{Score}_j$ proportionally without altering its dimension. Candidates whose residual directions align with the selected token are thereby progressively suppressed, and the process continues until the budget $K$ is reached.


% \subsection{Theoretical Analysis}

% \textbf{Why Does Cross-Modal Absorption Emerge?}
% \label{sec:why_absorption}

% Cross modal absorption arises from the information flow in autoregressive VLMs.
% Since post image text tokens can access visual tokens under causal attention and are typically used to produce final logits, visual information is progressively injected into text representations:
% \begin{equation}
% T^{l+1}
% =
% T^l
% +
% A_{TV}^l V_{\mathrm{vis}}^l
% +
% \Delta_T^l .
% \end{equation}
% Here, $A_{TV}^l V_{\mathrm{vis}}^l$ denotes the visual information received by text tokens.
% As depth increases, the text subspace absorbs more visual directions, increasing the projected energy of visual tokens and thus raising CMA.
% Details are provided in Appendix~\ref{app:cross_modal_absorption}.

% \paragraph{Complexity Analysis.}
% \label{sec:complexity}
% The extra overhead of SIEVE mainly comes from CMR projection and residual-space selection at pruning layers.
% Let $N_v$ be the number of visual tokens, $N_t$ the number of post-image text tokens, $d$ the hidden dimension, and $k$ the number of retained tokens.
% The scoring complexity of one pruning layer is:
% \begin{equation}
% \begin{aligned}
% C_{\mathrm{score}}
% =
% O\bigl(
% &N_t^2d + N_t^3 + N_vN_td \\
% &+ N_vN_t^2 + N_v^2d + kN_v
% \bigr).
% \end{aligned}
% \end{equation}
% The dominant cost usually comes from the residual-space Gram term $N_v^2d$.
% Since scoring is performed only at a few pruning layers, the overall overhead remains lightweight.
% A detailed analysis is provided in Appendix D.




==> Sections_Related_Work.tex <==
\section{Related Work}\label{Related Work}
\subsection{Multimodal Large Language Models}
VLMs perform multimodal reasoning by feeding visual and text tokens into LLMs.
Early systems use cross-attention or query-based designs, e.g.,
Flamingo~\cite{alayrac2022flamingo}, BLIP-2~\cite{li2023blip},
Kosmos-1~\cite{huang2023kosmos}, and PaLM-E~\cite{driess2023palme}, followed by
instruction-tuned models such as MiniGPT-4~\cite{zhu2023minigpt4},
mPLUG-Owl~\cite{ye2023mplugowl}, LLaVA~\cite{liu2023llava}, and
InstructBLIP~\cite{dai2023instructblip}. Recent high-resolution, general-purpose
VLMs such as Qwen-VL~\cite{bai2023qwen}, InternVL~\cite{chen2024internvl},
Gemini~\cite{team2023gemini}, LLaVA-NeXT~\cite{liu2024llavanext}, and
Qwen2.5-VL~\cite{bai2025qwen2} further improve OCR, grounding, and visual
reasoning, and extend to video understanding~\cite{maaz2024video-chatgpt,lin2024video-llava,li2024llavaonevision,li2024videochat2}.
However, high-resolution images, multi-image inputs, and long videos rapidly
inflate visual-token counts, incurring heavy self-attention and KV-cache
overhead; low-loss visual token compression is thus crucial for their efficient
inference.
\subsection{Visual Token Compression for VLMs}
Existing methods mainly fall into two categories. \textit{Attention-score
pruning}~\cite{chen2024FastV,zhang2025sparsevlm,xing2024pyramiddrop,liu2025dynamicllava}
removes low-importance tokens without training, but attention scores are biased
and unreliable indicators of true importance. \textit{Similarity-based
reduction}~\cite{bolya2023tome,wen2025dart,yang2025visionzip,shang2024prumerge,li2024tokenpacker}
merges similar tokens to preserve visual coverage, yet similarity need not
correspond to text-query relevance. Other methods use diversity- and
coverage-based selection~\cite{alvar2025divprune,zhang2025cdpruner,deng2025scope,holov},
adaptive token dropping~\cite{chen2026v2drop}, cross-modal information
flow~\cite{lin2025vtw,huang2025topv} or objective-driven~\cite{zhang2026trio}. These criteria, however, capture only a
single-layer local state and lack a holistic view of the multimodal reasoning
process. We therefore revisit the VLM inference process and find that, as layers deepen, text tokens progressively absorb visual information, reducing the independent contribution of some visual tokens. This suggests that token retention should focus on the residual information unexplained by text.
